Proof Pad: A New Development Environment for ACL2

Most software development projects rely on Integrated Development Environments (IDEs) based on the desktop paradigm, with an interactive, mouse-driven user interface. The standard installation of ACL2, on the other hand, is designed to work closely with Emacs. ACL2 experts, on the whole, like this mode of operation, but students and other new programmers who have learned to program with desktop IDEs often react negatively to the process of adapting to an unfamiliar form of interaction. This paper discusses Proof Pad, a new IDE for ACL2. Proof Pad is not the only attempt to provide ACL2 IDEs catering to students and beginning programmers. The ACL2 Sedan and DrACuLa systems arose from similar motivations. Proof Pad builds on the work of those systems, while also taking into account the unique workflow of the ACL2 theorem proving system. The design of Proof Pad incorporated user feedback from the outset, and that process continued through all stages of development. Feedback took the form of direct observation of users interacting with the IDE as well as questionnaires completed by users of Proof Pad and other ACL2 IDEs. The result is a streamlined interface and fast, responsive system that supports using ACL2 as a programming language and a theorem proving system. Proof Pad also provides a property-based testing environment with random data generation and automated interpretation of properties as ACL2 theorem definitions.

==> eptcsdata.tex <==
\providecommand{\firstpage}{13}
\providecommand{\publicationstatus}{R. Gamboa and J. Davis (Eds.): ACL2 Workshop 2013 (ACL2 '13).\\
EPTCS 114, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.114.2}{10.4204/EPTCS.114.2}}
\pdfoutput=1

